Local and Nonlocal Thermal Field Theory

Firstly, nonlocal field theories will be motivated, primarily in the gravity sector. We discuss how nonlocal theories of gravity can circumvent typical problems of finitely-many higher derivative theories and can, among other things, be either ghostfree and (potentially) renormalizable and yield a non-singular Newtonian potential. Afterwards we motivate finite temperature field theory, also known as thermal field theory, and study the thermodynamic behavior of both a local and a nonlocal scalar field theory. We compute (primarily leading-order) thermal corrections to the partition function for in low- and high- temperature expansions and calculate the thermal mass which is acquired through continuous interactions with the heat bath. We prove that the nonlocality does not contribute to the partition function of the free nonlocal theory. The presence of the nonlocality can only be noticed through interactions and we conclude that the partition function of the local and the nonlocal scalar theory are fundamentally different when interactions are included. We explain from both a mathematical and physical point of view why the nonlocality can only be noticed at the level of interactions and conclude that this cannot be generalized to arbitrary nonlocal modifications -- only those which do not introduce new poles in the propagator. We study whether our results can be reconciled with the stringy thermal duality and the conjectured Hagedorn phase and conclude that the former is violated, while Hagedorn behavior emerges in the high temperature expansion of the nonlocal scalar theory. We will interpret all these results.

==> TFTIDG.tex <==
\chapter{Towards thermal field corrections in the scalar IDG model \label{chaptertoymodelfinitet}}
Several temperature regimes are worth exploring and would, expectedly, contain totally different physics.
The interesting regimes are $T < M < M_{\text{p}}$, $ M > T > M_{\text{p}}$ and the very high temperature limit: $M < M_{\text{p}} < T$ where predominantly stringy states contribute to the partition function according to Atick and Witten's conjectured Hagedorn phase\ref{wittenatick}, \ref{wittenatick2}. The nonlocal kinetic term 
\begin{equation}\label{key}
S_0 = \frac{1}{2} \int d^4x \phi \square a(\square) \phi
\end{equation}
which contains $a(\square ) = \exp[-\square/M^2]$
has already been studied in chapter \ref{chapternonlocalfield} and
should recover the results from local field theory in the low-temperature regime. 
A priori, we do not know which corrections arise due to the interaction term 
of the IDG scalar toy model 
\begin{equation}\label{intaction}
S_{\text{int}} = \frac{1}{4M_{p} }\int d^{4}x \Bigg( 	\phi \partial_{\mu} \phi \partial^{\mu} \phi + \phi \square \phi a (\square) \phi - 
\phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi	\Bigg),
\end{equation}
because
this action contain \emph{derivative interactions}.
To the best of my knowledge, thermal field theory with derivative interactions has not been studied before in the literature which makes this an interesting academic enterprise.
\nnn
The thermal corrections for the scalar toy model have not been finished, the results will be deferred to an article which will hopefully be published in the near future. In this appendix, we will describe how derivative interactions can be dealt with in finite temperature field theory and preliminary steps on how to compute the lowest-order Feynman diagrams in the perturbative expansions will be provided in the next subsections.
\section{T $<$ M}
Both the free and interaction action
simplify considerably in the local $T < M$ regime. The free action reduces to an ordinary scalar theory
\begin{subequations} \label{laglag}
	\begin{equation}\label{sfree}
	S_{\text{free}} 
	= 
	\frac{1}{2} \int \ d^{4}x \ \phi \square  \phi, 
	\end{equation}
	while the interaction term contains no derivative interactions in this regime
	\begin{equation}\label{derivativeinteractions}
	\begin{aligned}
	S_{\text{int}} &= \frac{1}{M_{p}} \int d^{4}x \Bigg( 	\frac{1}{4}\phi \partial_{\mu} \phi \partial^{\mu} \phi 
	+ \frac{1}{4}\phi \square \phi a (\square) \phi - \frac{1}{4} \phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi	\Bigg) \\
	&= \frac{1}{4M_{p}} \int d^{4}x \Bigg( 	
	\phi \partial_{\mu} \phi \partial^{\mu} \phi 
	+ \phi \square \phi  \phi 
	- \phi \partial_{\mu} \phi \partial^{\mu} \phi	\Bigg) \\
	&= \frac{1}{ 4 M_{p} } \int d^{4}x \	
	\phi \square \phi^{  2}.
	\end{aligned}
	\end{equation}
\end{subequations}
The vertex factor $\mathcal{V}$ can be obtained trivially from the Lagrangian when considering a $\lambda \phi^4$ model, the derivative interactions of Eq. \ref{derivativeinteractions} however impede a straightforward identification of $\mathcal{V}$. The vertex factor $\mathcal{V} (p_1, p_2, p_3)$ for this nonlocal toy model has already been derived in \ref{UV} and the vertex factor at finite temperature is simply related to the ordinary vertex factor via a Wick rotation. The derivation is provided below
\subsubsection*{Vertex factor}
The vertex factor needs to be determined for the following action in the $T < M$ regime: 
\begin{equation}\label{key}
\begin{aligned}
S_{\text{int}} &= \frac{1}{ 4 M_{p} } \int_{X}	
\phi(\mathbf{x}, \tau) \square \phi^{  2}(\mathbf{x}, \tau) 
= - \frac{1}{ 2 M_{p} } \int_{X} \ g^{\mu \nu}	
\phi(\mathbf{x}, \tau) \partial_{\mu} \phi(\mathbf{x}, \tau) \partial_{\nu} \phi(\mathbf{x}, \tau).
\end{aligned}
\end{equation}
The trick is to Fourier transform the scalar fields using Eq. \ref{fourier} 
\begin{equation}\label{Svertex}
\begin{aligned}
S_{\text{int}} &= - \frac{\beta V}{ 2 M_{p} } \sum_{n = -\infty}^{\infty} \sum_{\mathbf{p}}
\sum_{i=1}^{3} \sum_{\substack{j = 1 \\ j \neq i}}^{3} 
\delta (\mathbf{p}_1 + \mathbf{p}_2  + \mathbf{p}_3)\ g^{\mu \nu}	
\phi_n(\mathbf{p}) (-i p_{i} ) \phi_n(\mathbf{p}) (-i p_{j} )  \phi_n(\mathbf{p}) \\
&=  \frac{\beta V}{  M_{p} } \sum_{n = -\infty}^{\infty} \sum_{\mathbf{p}} \delta (\mathbf{p}_1 + \mathbf{p}_2  + \mathbf{p}_3)\ g^{\mu \nu}	
\phi_n(\mathbf{p}) \phi_n(\mathbf{p}) (p_{1} \cdot p_2 + p_2 \cdot p_3 + p_1 \cdot p_3 )  \phi_n(\mathbf{p}) \\
&=  \frac{\beta V}{  M_{p} } \sum_{n = -\infty}^{\infty} \sum_{\mathbf{p}} \delta (\mathbf{p}_1 + \mathbf{p}_2  + \mathbf{p}_3)\ g^{\mu \nu}	
\phi_n(\mathbf{p}) \phi_n(\mathbf{p}) (p_{1} \cdot p_2 + p_2 \cdot p_3 + p_1 \cdot p_3 )  \phi_n(\mathbf{p}). \\
\end{aligned}
\end{equation}
The combined incoming four-momenta $k_1, k_2, k_3$ are conserved, \emph{i.e.}
\begin{equation}\label{key}
p_{1} + p_{2} + p_{3} = 0,
\end{equation}
which entails that
\bse
\begin{align}
& \ 	p_{1} \cdot p_2 + p_2 \cdot p_3 + p_1 \cdot p_3 \label{p11} \\
= & \ p_{1} \cdot \left(-p_1 - p_3 \right) + p_2 \cdot \left(-p_1 - p_2 \right) + \left(-p_2 - p_3 \right) \cdot p_3 \nonumber \\
= & -p_{1}^2 -p_{2}^2 -p_{3}^2 - \left[ p_{1} \cdot p_{2} + p_{2} \cdot p_{3} + p_{3} \cdot p_{1} \right] \label{p13}. 
\end{align}
\ese
The equivalence of Eqs. \ref{p11} and \ref{p13} implies that 
	\begin{equation}\label{key}
p_{1} \cdot p_{2} + p_{2} \cdot p_{3} + p_{1} \cdot p_{3} = - \frac{1}{2} \left[ p_{1}^2 + p_{2}^2 + p_{3}^2 \right]
	\end{equation}
and	consequently the interactions are described by
\begin{equation}\label{key}
S_{\text{int}}  =  - \frac{ \beta V}{ 2  M_{p} } \sum_{n = -\infty}^{\infty}  g^{\mu \nu}	
\phi_n(\mathbf{p}) \phi_n(\mathbf{p}) (p_1^2 + p_2^2 + p_3^2)
\phi_n(\mathbf{p}),
\end{equation}
from which the corresponding vertex factor can be deduced
\begin{equation}\label{vertexlocal}
\frac{1}{M_p} \mathcal{V} (p_1, p_2, p_3) = -  \frac{ \beta V}{ 2 M_p} (p_{1}^2 + p_2^2 +  p_3^2 ).
\end{equation}






\subsubsection{Thermal corrections}
An even number of fields is required in order to perform Bloch-De Dominicis contractions, so the lowest-order non-vanishing correlation functions are given by 
\begin{subequations}
	\begin{equation}\label{key}
	\begin{aligned}
	\ln \mathcal{Z}_2 &= 
	\frac{1}{2} \expval{S_I^2}
	=
	\frac{1}{2} \left( -  \frac{ \beta V}{ 2 M_p} \right)^{2}
	\int_{X} \int  \mathcal{D} \tilde{\phi} \
	\frac{  e^{S_0} \tilde{\phi}^6 (p_{1}^2 + p_2^2 +  p_3^2 )^{2}}{  e^{S_0} } \\
	&=
	\frac{ \beta^2 V^2}{ 8 M_p^2}  \int_{X} 
	\sum_{n_1, ... , n_6}
	\sum_{\mathbf{p}_{1}, ... , \mathbf{p}_{6}}
	\frac{\beta^2}{V^2}
	\exp[i (\mathbf{p}_{1} + ... + \mathbf{p}_{6}) \cdot \mathbf{x} ]
	\exp[i (\omega_{n_{1}} + ... + \omega_{n_{6}}   ) \tau ]  (p_{1}^2 + p_2^2 +  p_3^2 )^{2} \frac{A}{B}, \\
	\end{aligned}
	\end{equation}
	where
	\begin{align}
	A &= \prod_{l} \prod_{\mathbf{q}} \int \mathcal{D} \tilde{\phi}_{l}(\mathbf{q}) 
	\exp \left[
	-\frac{1}{2} \beta^2 (\omega_l^2 + \mathbf{q}^2)
	\tilde{\phi}_{l}(\mathbf{q}) 
	\tilde{\phi}_{- l}(- \mathbf{q})
	\right]
	\cdot
	\tilde{\phi}_{n_{1}}(\mathbf{p}_{1}) 
	\cdots
	\tilde{\phi}_{n_{6}}(\mathbf{p}_{6}),\\
	B &= \prod_{l} \prod_{\mathbf{q}} \int \mathcal{D} \tilde{\phi}_{l}(\mathbf{q}) 
	\exp \left[
	-\frac{1}{2} \beta^2 (\omega_l^2 + \mathbf{q}^2)
	\tilde{\phi}_{l}(\mathbf{q}) 
	\tilde{\phi}_{- l}(- \mathbf{q})
	\right].
	\end{align}
\end{subequations}
The integral factorizes into a product of three Gaussian integrals and has a combinatorial factor of $(6 - 1)!! = 15$.
The only first-order loop is
\begin{equation}\label{feynmandiagram}
\ln \mathcal{Z}_2 = 15 \	
\begin{tikzpicture}[baseline=(v3), node distance=1cm and 1cm]
\begin{feynman}[inline=(v3)]
\coordinate[] (v1);
\coordinate[vertex, right=of v1] (v2);
\coordinate[vertex, right=of v2] (v3);
\coordinate[right=of v3] (v4);
\draw[fermion,
momentum'=\(\mathbf{k}\)] (v1) --  (v2);
\semiloop[fermion]{v2}{v3}{0}[$(\mathbf{k} + \mathbf{p}, \omega_k + \omega_{p})$];
\semiloop[fermion]{v3}{v2}{180}[$(\mathbf{p},  \omega_{p})$][below];
\draw[fermion, momentum'=\(\mathbf{k}\)] (v3) -- (v4);
\end{feynman}
\end{tikzpicture}
= 15 \	
\begin{tikzpicture}[baseline=(v3), node distance=1cm and 1cm]
\begin{feynman}[inline=(v3)]
\coordinate[] (v1);
\coordinate[vertex, right=of v1] (v2);
\coordinate[vertex, right=of v2] (v3);
\coordinate[right=of v3] (v4);
\draw[fermion,
momentum'=\(\mathbf{k}\)] (v1) --  (v2);
\semiloop[fermion]{v2}{v3}{0}[$(\mathbf{q}, \omega_q)$];
\semiloop[fermion]{v3}{v2}{180}[$(\mathbf{q} - \mathbf{k},  \omega_{q} - \omega_k)$][below];
\draw[fermion, momentum'=\(\mathbf{k}\)] (v3) -- (v4);
\end{feynman}
\end{tikzpicture},
\end{equation}
where both momentum and Matsubara modes have been given new indices in the last step.
In order to evaluate this diagram, the following frequency sum needs to be computed
\begin{equation}\label{key}
\bal
S(i \omega_n)
&=
T
\sum_{\omega_q, \omega_k}
\mathcal{D}(i \omega_q, \maq)
\mathcal{D}(i(\omega_q - \omega_k), \maq - \mathbf{k}) \\
&= \frac{1}{\beta} \sum_{\omega_q, \omega_k} \frac{1}{\omega_q^2 + E_{\maq}^2} 
\frac{1}{(\omega_q - \omega_k)^2 + E_{\maq - \mathbf{k}}^2}.
\eal
\end{equation}
%We can get rid of one of these variables by choosing $p_1 = -p_2$, $p_3 = 0$, implying that
%\begin{equation}\label{key}
%\frac{1}{M_p} \mathcal{V} (p_1, p_2, p_3) = -  \frac{ \beta V}{ M_p} p_{1}^2.
%\end{equation}
This frequency sum is performed in Appendix \ref{freqsumappendix} and yields
\begin{equation}\label{key}
\bal
S(i\omega_m, \map) = - \frac{1}{4E_1 E_2} 
\Bigg[
&\left[1 + n_1 + n_2
\right]
\left[ \frac{1}{ i \omega - E_1 - E_2}  - \frac{1}{ i \omega + E_1 + E_2}  
\right] \\
&+ \left[-n_1 + n_2\right]
\left[\frac{1}{ i \omega - E_1 + E_2}
-
\frac{1}{ i \omega + E_1 - E_2}
\right]
\Bigg],
\eal
\end{equation}
where $n_i$ is related to the Bose-Einstein distribution function through
$$n_i = n(E_i) = \frac{1}{e^{\beta E_i} - 1}$$
and $\omega$ is the Matsubara frequency of the external line.
Note that the weights $n_1$ and $n_2$ involve the on-shell energy of the internal line of the diagram. Furthermore, combining the definition of energy
\begin{subequations}
	\begin{equation}
	E = \sqrt{m^2 + \mathbf{p}^2} 
	\end{equation}
	with the kinematics one obtains the following energies for the massless gravitons
	\begin{equation}
	E_1 =  \sqrt{m_1^2 + \mathbf{q}} = q, \ \ \ \ \ E_2 = \sqrt{m_2^2 + (\mathbf{q} - \mathbf{k})^2 } = q - k.
	\end{equation}
\end{subequations}
The contribution to the partition function from the first-order loop diagram is given by


$$
\bal
\ln \mathz_2 =  
- \frac{ \beta^3 V^2}{ 32 M_p^2} \int \frac{d^3q}{(2 \pi)^3}  \frac{\left[k^2 + q^2 + (q-k)^2 \right]^2}{E_1 E_2}
&\Bigg[
\left[1 + n_1 + n_2
\right]
\left[ \frac{1}{ i \omega - E_1 - E_2}  - \frac{1}{ i \omega + E_1 + E_2}  
\right] \\
& \ \ + \left[-n_1 + n_2\right]
\left[\frac{1}{ i \omega - E_1 + E_2}
-
\frac{1}{ i \omega + E_1 - E_2}
\right]
\Bigg]
\eal
$$
$$
\bal
\ \ \ \ \ \ \ \ =
- \frac{ \beta^3 V^2}{ 64 \pi^2 M_p^2} \int_0^\infty dq  \frac{
	\left[2(q - k)^2 + 2qk \right]^2}{q[q-k]}
\Bigg[&
\left[1 + [e^{\beta q} - 1]^{-1} + [e^{\beta (q-k)} - 1]^{-1}
\right] \cdot \left[ \frac{1}{ i \omega - 2q + k}  - \frac{1}{ i \omega + 2q - k}  
\right] \\
& \ \  + \left[ [e^{\beta (q-k)} - 1]^{-1} -[e^{\beta q} - 1]^{-1}\right] \cdot \left[\frac{1}{ i \omega - k}
-
\frac{1}{ i \omega + k}
\right]
\Bigg]
\eal \\
$$
\begin{equation}
\label{T<Mcorrection}
\bal
\ \ \ \ \ \ \ \ = 
- \frac{ \beta^3 V^2}{ 32 \pi^2 M_p^2} \int_0^\infty dq  
	\left[1  - \frac{k}{q} + \frac{k}{q-k} \right]^2
&\Bigg[
\left[\frac{e^{\beta q}}{e^{\beta q} - 1} + \frac{e^{\beta k}}{e^{\beta q} - e^{\beta k}}
\right]  \left[ \frac{1}{ i \omega - 2q + k}  - \frac{1}{ i \omega + 2q - k}  
\right] \\
& \ \ + \left[ \frac{1}{e^{\beta (q-k)} - 1} -\frac{1}{e^{\beta q} - 1} \right]  \left[\frac{1}{ i \omega - k}
-
\frac{1}{ i \omega + k}
\right]
\Bigg].
\eal \\
\end{equation}
We will first
look at the limit of \emph{vanishing external momenta}, as these diagrams are mathematically easier to deal while these can nonetheless indicate whether the corresponding Feynman diagram will or will not converge.
A tedious computation of 48 integrals can be circumvented by ``cutting off the external momenta'', that is to say: set $k = 0$ in the Feynman diagram displayed in Eq. \ref{feynmandiagram}. The external momenta can be reintroduced after having computed the simplified integrals.
\subsubsection*{1-loop, 2-point function with zero external momenta}
The one-loop correction to the partition function can be rewritten as a relatively simple integral in the absence of external momenta. Setting $k = \omega = 0$ in Eq. \ref{T<Mcorrection} gives
\begin{equation}\label{lnmathz2}
\bal
\ln \mathz_2 &= 
 \frac{ \beta^3 V^2}{32 \pi^2 M_p^2} \int_0^\infty   
\frac{dq}{q}
\frac{e^{\beta q} + 1}{e^{\beta q} - 1 }
\stackrel{(z=\beta q)}{=} 
\frac{ \beta^3 V^2}{32 \pi^2 M_p^2} \int_0^\infty   
\frac{dz}{z}
\frac{e^{z} + 1}{e^{z} - 1 }  \\  
\eal 
\end{equation}
which has a second order pole at $z=0$. 
The 1-loop 2-point function at zero temperature is UV-divergent and the result is in complete accordance with the analysis of superficial degree of
divergence according to which the non-locality does not
affect the integrals at at 1-loop level. There, the divergence structure is exactly the same as that of GR at 1-loop \ref{UV}. I recall the important feature of thermal field theory that no additional UV-divergences can emerge at finite temperature due to the exponential suppression of the distribution functions.
\nnn
Let us get back to Eq. \ref{lnmathz2}:
this integral is infared divergent and therefore needs to be regulated.  We can introduce a Schwinger parameter $\alpha$ and rewrite the integral as
\begin{equation}\label{key}
 \int_{z}^{\infty} d\alpha \int_0^\infty
\frac{ e^{-z} + 1}{ e^{-z} - 1} e^{-z \alpha} dz.
\end{equation}
%The standard integral
%\begin{equation}\label{key}
%\bal
%\int_0^\infty  \frac{dz}{z}
%\frac{e^{z} + 1}{e^{z} - 1 } &= \frac{1}{2}\int_{-\infty}^\infty  \frac{dz}{z}
%\frac{e^{z} + 1}{e^{z} - 1 } 
%= \frac{1}{2} (2\pi i) \lim_{z \rightarrow 0}\frac{d}{dz}  
%\frac{z (e^{z} + 1)}{e^{z} - 1 } \\ 
%&= \frac{1}{2} (2\pi i) \lim_{z \rightarrow 0} 
%\frac{(e^{z} + 1 + ze^z) (e^{z} - 1) - ze^{z} (e^{z} + 1) }{ (e^{z} - 1)^2 }
% = \pi i
% \eal
%\end{equation}
\section{T $>$ M}
Nonlocal phenomena emerge at $T \geq M$, where the exponential damping of $a(\square)$ can no longer be neglected. It would be interesting to investigate whether the scalar infinite-derivative theory obeys the Hagedorn conjectures, \emph{i.e.} whether the partition function satisfies $\mathz(T) \sim (T^3 - T)$ for temperatures above the scale of nonlocality.

\subsubsection*{Vertex factor}
We obtain a more complicated vertex factor than in the local case, \emph{i.e.} Eq. \ref{vertexlocal}, since $\frac{1}{4}\phi \square \phi a (\square) \phi$ and $- \frac{1}{4} \phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi$ contribute to the vertex factors as well. Furthermore, the vertex factor that we obtained in \ref{vertexlocal} is divided by $(-2)$ since 
$\frac{1}{4} \phi \square \phi^2 =
\frac{1}{2} \phi^2 \square \phi
=
-\frac{1}{2}\phi \partial_\mu \phi \partial^{\mu} \phi $, while the new local interacting term is $\frac{1}{4}\phi \partial_\mu \phi \partial^{\mu} \phi $. The remaining contributions to the vertex factor are as follows:

$$
\frac{1}{4} 
\big[ \phi \square \phi a (\square) \phi -  \phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi \big]
=
\frac{1}{4} \left[ \phi \square  \phi a (\square) \phi 
- g^{\mu \nu} \phi \partial_{\mu} \phi a(\square)\partial_{\nu} \phi \right].
$$
Let us now examine the second and third terms, i.e. $\frac{1}{4} \phi \square \phi a(\square) \phi$ and $-\frac{1}{4} \phi \partial_{\mu} \phi a(\square) \partial^{\mu} \phi$. In momentum space they read
\begin{equation}\label{key}
-\frac{1}{4} \phi k_{\mu}k^{\mu} \phi a(\square) \phi \ \ \ \ \ \ \ \ \text{and} \ \ \ \ \ \ \ \ \frac{1}{4} \phi k_{\mu} \phi a(k_{\mu}k^{\mu}) k^{\mu} \phi
\end{equation}
When calculating the equation of motion for $k_1$, the left term contributes (multiplied by i to get the vertex factor):
$$\frac{1}{4}(k_3 \cdot k_1 + k_1 \cdot k_2) e^{\bar{k}_{1}^{2}} \ ,$$
and the right Term
$$-\frac{1}{4}(-k_2 \cdot k_2 - k_3 \cdot k_3) e^{\bar{k}_{1}^{2}} = -\frac{1}{4}(-k_2^2 - k_3^2) e^{\bar{k}_{1}^{2}} \ ,$$
\begin{equation}\label{ver1}
\begin{aligned}
\frac{1}{4}(k_3 \cdot k_1 + k_1 \cdot k_2 - k_3^2 - k_2^2) \exp(\bar{k}_{1}^{2}) &= \frac{\exp(\bar{k}_{1}^{2})}{4}((-k_1 - k_2) \cdot k_1 + k_1 \cdot k_2 - k_3^2 - k_2^2)  = \frac{\exp(\bar{k}_{1}^{2})}{4}(- k_3^2 - k_2^2 - k_1^2) \\
&= -\frac{\exp(\bar{k}_{1}^{2})}{4}( k_3^2 + k_2^2 + k_1^2) 
\end{aligned}
\end{equation}
Similarly, we obtain
\begin{equation}\label{ver2}
\frac{1}{4}(k_3 \cdot k_2 + k_2 \cdot k_1 - k_1^2 - k_3^2)e^{\bar{k}_{2}^{2}} = \frac{1}{4}((k_1 - k_2) \cdot k_2 + k_2 \cdot k_1 - k_1^2 - k_3^2)e^{\bar{k}_{2}^{2}} = -\frac{1}{4}(k_1^2 + k_{2}^{2} +  k_3^2)e^{\bar{k}_{2}^{2}} \ ,
\end{equation}
\begin{equation}\label{ver3}
\frac{1}{4}(k_1 \cdot k_3 + k_3 \cdot k_2 - k_2^2 - k_1^2)e^{\bar{k}_{3}^{2}} = \frac{1}{4}((-k_2 - k_3) \cdot k_3 + k_3 \cdot k_2 - k_2^2 - k_1^2)e^{\bar{k}_{3}^{2}} = -\frac{1}{4}(k_1^2 + k_{3}^{2} +  k_3^2)e^{\bar{k}_{3}^{2}} \ .
\end{equation}
The vertex factor can thus be written as
\begin{equation}\label{key}
V(k_1, k_2, k_3) = C(k_1, k_2, k_3)\Bigg[1 - \exp(\bar{k}_1^{2}) - \exp(\bar{k}_2^{2}) - \exp(\bar{k}_3^{2})\Bigg] \ .
\end{equation}




When we collect the $e^{\bar{k}_1^2}$ terms, we obtain the following vertex factor:
\begin{equation}\label{key}
\begin{aligned}
& =
\frac{1}{4} \left( k_3 \cdot k_1 + k_1 \cdot k_2 - k_3^2 - k_2^2 \right) e^{\bar{k}_1^2} = -\frac{1}{4} \left( k_1^2 +  k_2^2 + k_3^2 \right) e^{\bar{k}_1^2},
\end{aligned}
\end{equation}
where we used the fact that the incoming momenta $k_1, k_2, k_3$ satisfy
$k_1 + k_2 + k_3 = 0$.
Similarly we obtain the remaining two contributions
$
-\frac{1}{4} \left( k_1^2 +  k_2^2 + k_3^2 \right) e^{\bar{k}_2^2}$ and  $ -\frac{1}{4} \left( k_1^2 +  k_2^2 + k_3^2 \right) e^{\bar{k}_3^2}$.
We have thus obtained the vertex factor
\begin{subequations}
	\begin{equation}\label{key}
	\frac{1}{M_p} \mathcal{V}(k_1, k_2, k_3 ) = \frac{1}{M_p} C(k_1, k_2, k_3) \left[
	1 - e^{\bar{k}_1^2} - e^{\bar{k}_2^2} - e^{\bar{k}_3^2}
	\right],
	\end{equation}
	where
	\begin{equation}\label{key}
	C(k_1, k_2, k_3) =  \frac{ \beta V}{ 4 } (k_{1}^2 + k_2^2 +  k_3^2 ).
	\end{equation}
Note that the vertex factor are exponentially enhanced, which means that the vertex factors become smeared out over a region of space-time at high energies and temperatures. \nnn	
We will encountered the squared vertex factor as well	\begin{equation}\label{V2}
	\mathcal{V}^{2}(k_1, k_2, k_3 ) =  C^{2}(k_1, k_2, k_3) \left[
	1 - 2 e^{ \bar{k}_1^2} - 2 e^{\bar{k}_2^2} - 2 e^{\bar{k}_3^2}
	+ 2 e^{ \bar{k}_1^2}  e^{ \bar{k}_2^2}
	+ 2 e^{ \bar{k}_2^2}  e^{ \bar{k}_3^2}
	+ 2 e^{ \bar{k}_3^2}  e^{ \bar{k}_1^2}
	+  e^{ 2 \bar{k}_1^2}
	+  e^{ 2 \bar{k}_2^2}
	+  e^{ 2 \bar{k}_3^2}
	\right]
	\end{equation}
\end{subequations}
The vertex factor simplifies significantly for the following choice of momenta $$k_1 = -k_2 = k, k_3 = 0,$$
where $k_3 = 0$ means that the external momenta are zero and $k_1 = -k_2$ entails that the magnitude of the four-momentum throughout the entire loop remains constant. Eq. \ref{V2} then reduces to
\begin{equation}\label{key}
\mathcal{V}^{2}(k, -k, 0) =   \frac{\beta^2 V^2}{4} C^2(k, -k, 0) [-2e^{\bar{k}^2}] 
=  \beta^2 V^2 k^4  e^{ 2 \bar{k}^2}.
\end{equation}

\subsubsection{Thermal corrections}
The first contributions from the interaction term to the partition function are given by $\frac{1}{2}\expval{S_{\text{I}}^2}$, where
\begin{equation}\label{key}
\begin{aligned}
S_{\text{I}}^{2} = \frac{1}{16 M_{p}^2} \int d^{4}x \Bigg[& 	\phi \partial_{\mu} \phi \partial^{\mu} \phi 
\phi \partial_{\mu} \phi \partial^{\mu} \phi 
+ 
\phi \square \phi a (\square) \phi 
\phi \partial_{\mu} \phi \partial^{\mu} \phi 
-  \phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi 
\phi \partial_{\mu} \phi \partial^{\mu} \phi \\
&+
\phi \square \phi a (\square) \phi 
\phi \partial_{\mu} \phi \partial^{\mu} \phi +
\phi \square \phi a (\square) \phi 
\phi \square \phi a (\square) \phi  
-  \phi \square \phi a (\square) \phi  
\phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi \\
&-  \phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi
\phi \partial_{\mu} \phi \partial^{\mu} \phi 
- \phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi
\phi \square \phi a (\square) \phi 
+  \phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi
\phi \partial_{\mu} \phi a(\square)\partial^{\mu} \phi \Bigg].
\end{aligned}
\end{equation}
Solely the following Feynman diagram gives contributions to $\ln \mathcal{Z}_2$
$$
\begin{tikzpicture}[baseline=(v3), node distance=1cm and 1cm]
\begin{feynman}[inline=(v3)]
\coordinate[] (v1);
\coordinate[vertex, right=of v1] (v2);
\coordinate[vertex, right=of v2] (v3);
\coordinate[right=of v3] (v4);
\draw[fermion,
momentum'=\(\mathbf{k}\)] (v1) --  (v2);
\semiloop[fermion]{v2}{v3}{0}[$(\mathbf{q}, \omega_q)$];
\semiloop[fermion]{v3}{v2}{180}[$(\mathbf{q} - \mathbf{k},  \omega_{q} - \omega_k)$][below];
\draw[fermion, momentum'=\(\mathbf{k}\)] (v3) -- (v4);
\end{feynman}
\end{tikzpicture}
$$
so the thermal corrections are computed similarly to in the $T<M$ regime where the same Feynman diagram appeared. The vertex term has however changed considerably compared to in the  $T<M$ regime. \nnn
The frequency sum for this Feynman diagram has been performed in Appendix \ref{freqsumappendix} and gives
\begin{equation}\label{key}
\bal
S(i\omega_m, \map) = - \frac{1}{4E_1 E_2} 
\Bigg[
&\left[1 + n_1 + n_2
\right]
\left[ \frac{1}{ i \omega - E_1 - E_2}  - \frac{1}{ i \omega + E_1 + E_2}  
\right] \\
&+ \left[-n_1 + n_2\right]
\left[\frac{1}{ i \omega - E_1 + E_2}
-
\frac{1}{ i \omega + E_1 - E_2}
\right]
\Bigg],
\eal
\end{equation}
where $n_i$ is related to the Bose-Einstein distribution function by
$$n_i = n(E_i) = \frac{1}{e^{\beta E_i} - 1}$$
and $\omega$ is the Matsubara frequency of the external line. This first order loop diagram will firstly be evaluated with zero external momenta.
\subsubsection*{1-loop, 2-point function with zero external momenta}
Setting $E_1 = E_2 = k$ and $\omega = 0$ gives
$$
\bal
\ln \mathz_2 =  -
 \frac{ \beta^2 V^2 }{ 64 M_p^2} \int \frac{ k^4}{E_1 E_2}  e^{ 2 \bar{k}^2}
&\Bigg[
\left[1 + n_1 + n_2
\right]
\left[ \frac{1}{ i \omega - E_1 - E_2}  - \frac{1}{ i \omega + E_1 + E_2}  
\right] \\
& \ \ + \left[-n_1 + n_2\right]
\left[\frac{1}{ i \omega - E_1 + E_2}
-
\frac{1}{ i \omega + E_1 - E_2}
\right]
\Bigg]
\eal
$$
$$
\ \ \ \ \ \ \ =  
\frac{ \beta^2 V^2 }{ 256 M_p^2} \int dk \ k  e^{ 2 \bar{k}^2} 
\left[\frac{e^{\beta k} + 1}{e^{\beta k} - 1} 
\right]
$$
This integral is both infrared and ultraviolet divergent, since 
the BE-distribution diverges for
$k \rightarrow 0$ and moreover
$\int_0^\Lambda dk \ ke^{2\bar{k}^2} \rightarrow \infty \ \ \text{for } \Lambda \rightarrow \infty$.
%We thus obtain
%\begin{equation}\label{key}
%\begin{aligned}
%\Gamma_2 &= \frac{1}{16 M_p^2} \int \ \frac{d^4 k}{(2 \pi)^4} \frac{V^2 (k) }{k^4} \\
%&= \frac{\beta^2 V^2}{ M_p} \int \ \frac{d^4 k}{(2 \pi)^4} \frac{(k_{1}^2 + k_2^2 +  k_3^2 )^2 }{k^4} \\
%&= \frac{\beta^2 V^2}{ 16 \pi^4 M_p} \int \ 4 \pi k_E^3 \sqrt{1 - x^2 } \frac{(k_{1}^2 + k_2^2 +  k_3^2 )^2 }{k^4} \ dx \ dk_E,
%\end{aligned}
%\end{equation}
%where $x$ is the cosine of the angle between $p_E$ and $k_E$.
\nnn
Theories of gravity are gauge theories since the graviton is known to have both spin-0 and spin-2 modes. Rather than having examined a full-fledged theory infinite derivative theory of gravity, a scalar toy model will be studied in the future to obtain insights into its finite temperature behavior. Critical evaluation as to whether these properties carry over to a gauge theory of gravity is essential in order to  determine the behavior of BGKM-theory at finite temperature.

